Extracting Einstein from the Loop-Level Double-Copy

The naive double-copy of (multi) loop amplitudes involving massive matter coupled to gauge theories will generically produce amplitudes in a gravitational theory that contains additional contributions from propagating antisymmetric tensor and dilaton states even at tree-level. We present a graph-based approach that combines the method of maximal cuts with double-copy construction to offer a systematic framework to isolate the pure Einstein-Hilbert gravitational contributions through loop level. Indeed this allows for a bootstrap of pure-gravitational results from the double-copy of massive scalar-QCD. We apply this to construct the novel result of the D-dimensional one-loop five-point QFT integrand relevant in the classical limit to generating observables associated with the radiative effects of massive black-hole scattering via pure Einstein-Hilbert gravity.

==> doubleCopyMC.tex <==
\section{The double copy}

==> methodOfMaximalCuts.tex <==
\section{Method of maximal cuts}

With the objective of building pure gravity amplitudes from double copies of QCD, we use the method of maximal cuts in a constructive way to project out unwanted states at the level of the numerator dressings. From {\color{red} OUR OTHER PAPER} we have a set of kinematic numerator dressings for amplitudes with gluons and massive scalar particles, which obey the color-kinematics duality. A `naive double copy'  dressing of the graph numerators in a gravitational theory is simply the square of these numerators 
\begin{equation}
n^G_g = \left(n^{QCD}_g \right)^2,
\end{equation}
where $g$ is a cubic graph topology contributing to the amplitude, and $n_g^{QCD}$ is the kinematic numerator dressing from the gauge theory amplitude. This dressing is naive in the sense that a pure double copy will not only have gravitons as internal states, but also axions and dilatons.

At both tree and loop level the method of maximal cuts decomposes amplitudes (and amplitude integrands) into products of tree amplitudes using generalized unitarity methods
\begin{equation}\label{Eq:GeneralUnitarityCut}
\mathcal{C}^{N^kMC} = \sum_{\text{states}}\mathcal{A}^{\text{tree}}_{m(1)}...\mathcal{A}^{\text{tree}}_{m(p)}\hspace{2cm}k \equiv\sum_{i=1}^p m(i)-3,
\end{equation}
where $\mathcal{A}^{\text{tree}}_{m(i)}$ are tree-level $m(i)$ multiplicity amplitudes, and $k$ is the number of propagators that remain off shell. For cuts of gravitational amplitudes, the tree amplitudes $\mathcal{A}^{\text{tree}}_{m(i)}$ are unordered. Missing contributions\footnote{or in this case excess contributions from states other than gravitons} are attributed to new higher-level contact terms as necessary. We perform the unitarity cuts for tree level amplitudes and loop level integrands in $D$ dimensions, and ensure that the only states running through the cut propagators are gravitons we use the $D$-dimensional graviton projector
\begin{equation}\label{Eq: Big gravity projector}
P^{\mu \nu \rho \sigma} (p,q) = \sum_{\text{pols.}}\varepsilon^{\mu \nu}(-p) \varepsilon^{\rho \sigma}(p) = \frac{1}{2} (P^{\mu \rho}P^{\nu \sigma} + P^{\mu \sigma} P^{\nu \rho}) - \frac{1}{D_s - 2} P^{\mu \nu}P^{\rho \sigma},
\end{equation}
where
\begin{equation}
P^{\mu \nu} = \eta^{\mu \nu} - \frac{q^{\mu} p^{\nu} + p^{\mu}q^{\nu}}{p \cdot q}.
\end{equation}
In some cases, when there are no massless triangles or bubbles contributing to the cut, we can use a simpler projector
\begin{equation}\label{Eq: Nice gravity projector}
\sum_{\text{pols.}} \varepsilon_{\mu \nu}(-p) \varepsilon_{\rho \sigma}(p) = \frac{1}{2} \eta_{\mu \rho} \eta_{\nu \sigma} + \frac{1}{2} \eta_{\mu \sigma} \eta_{\nu \rho} - \frac{1}{D_s - 2} \eta_{\mu \nu} \eta_{\rho \sigma}.
\end{equation}

We begin by performing the maximal cuts of all topologies contributing to the amplitude, and comparing with the sewn tree amplitudes. In the maximal cuts all propagators are put on-shell. This in turn means that all the tree amplitudes in Equation~\ref{Eq:GeneralUnitarityCut} are three-point amplitudes, and only one graph contributes to each cut. The discrepancy between the cut graphs and the sewn trees is attributed to other states than the gravitons running through the cut, and is given by 
\begin{equation}
{n_D}_g = \mathcal{C}_g^{G} - \sum_{\text{states}}\mathcal{A}^{\text{tree}}_{3, 1}...\mathcal{A}^{\text{tree}}_{3, i},
\end{equation}
where $\mathcal{C}_g^{G}$ is the maximal cut of  the fully dressed graph topology $g$. This term is then symmetrized according to the isomorphisms of the graph topology $g$, and subtracted from the numerator dressing of the graph
\begin{equation}
n^{G, \text{updated}}_g = (n_g^{QCD})^2 -  {n_D}_g.
\end{equation}

The remaining cuts ($N^kMC$) are then performed systematically until no more information can be gained, beginning with the next-to-maximal cuts, $NMC$. Here, all but one propagator are put on shell. Similarly, for the $N^2MC$ two propagators are held off-shell, and so on. In this paper, the graviton numerators can be determined by performing all cuts up to and including the $N^2MC$. However, it is useful to skip some ill-defined cuts at $NMC$ and $N^2MC$ and extract the information using $N^3MC$, as described in the next section.
